Automating Source Code Refactoring in the Classroom

Refactoring is the practice of improving software quality without altering its external behavior. Developers intuitively refactor their code for multiple purposes, such as improving program comprehension, reducing code complexity, dealing with technical debt, and removing code smells. However, no prior studies have exposed the students to an experience of the process of antipatterns detection and refactoring correction, and provided students with toolset to practice it. To understand and increase the awareness of refactoring concepts, in this paper, we aim to reflect on our experience with teaching refactoring and how it helps students become more aware of bad programming practices and the importance of correcting them via refactoring. This paper discusses the results of an experiment in the classroom that involved carrying out various refactoring activities for the purpose of removing antipatterns using JDeodorant, an Eclipse plugin that supports antipatterns detection and refactoring. The results of the quantitative and qualitative analysis with 171 students show that students tend to appreciate the idea of learning refactoring and are satisfied with various aspects of the JDeodorant plugin's operation. Through this experiment, refactoring can turn into a vital part of the computing educational plan. We envision our findings enabling educators to support students with refactoring tools tuned towards safer and trustworthy refactoring.

==> Sections/07_Threats.tex <==
\vspace{-.2cm}
\section{Threats to Validity}
\label{Section:Threats}

This section discusses the threats that could affect the validity of our experiment. Concerning the success of the assignment to enable students to better understand the application of refactoring, students' performance is measured by \hl{only one} assignment. It is possible that other factors contributed to the success of the experiment such as previous work experience. Further, the assignment relies on one refactoring recommendation tool, which may raise concerns about the generalizability of the results. However, the JDeodorant tool is available with an education license to identify antipatterns and recommend refactoring. The assignment can be reused with other quality assessment tools as well upon their availability.


==> Tables/Project.tex <==
\begin{table}
  \centering
  %\fontsize{8}{9}\selectfont
	%\tabcolsep=0.05cm
	 \caption{The list of open-source projects used in the assignment.}
	 \label{Table:Project}
%\begin{sideways}
\begin{adjustbox}{width=0.48\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lclllll}\hline
\toprule
\bfseries Project & \bfseries \# commits &  \bfseries  \# contributors & \bfseries Domain   \\
\midrule
Ant & 14,887 & 64 & Java builder \\
GanttProject & 4,361 & 38 & Project management\\
JCommander & 1,009 & 64 & Command line parsing\\ 
JFreeChart & 4,218 & 24 & Data visualization \\
JHotDraw & 804 & 3 & Data visualization \\
Log4J & 12,211 & 137 & Logging\\
Nutch & 3,293 & 46 & Web crawler\\
Rihno & 4,119 & 80 & Script builder \\
Xerces &  6,463 & 5 & XML parser \\



\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\vspace{-.3cm}
\end{table}

%https://github.com/apache/ant
%https://github.com/jfree/jfreechart
% https://github.com/apache/nutch
% https://github.com/apache/logging-log4j2
% https://github.com/mozilla/rhino
% https://github.com/apache/xerces-c
% https://github.com/cbeust/jcommander
% https://github.com/bardsoftware/ganttproject
%https://sourceforge.net/projects/jhotdraw/


==> Tables/RelatedWork.tex <==





\begin{table}
  \centering
  %\fontsize{8}{9}\selectfont
	%\tabcolsep=0.05cm
	 \caption{Related work in refactoring in education.}
	 \label{Table:Related_Work_in_education}
%\begin{sideways}
\begin{adjustbox}{width=0.5\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lclllll}\hline
\toprule
\bfseries Study & \bfseries Year &  \bfseries  Teaching method &  \bfseries Tool   \\
\midrule
Smith \etal \cite{smith2006innovative} & 2006 & Incremental learning & N/A \\
Stoecklin \etal \cite{stoecklin2007teaching} & 2007 & Incremental learning & N/A \\
Rabb \cite{raab2012codesmellexplorer} & 2012 & Visualization/Gamification & CodeSmellExplorer \\
Lobez \etal \cite{lopez2014design} & 2014 & E-activity planning & N/A \\
Abid \etal \cite{abid2015reflections} & 2015 & Experimentation & SonarQube/FindBugs \\
& & & PMD/SourceMonitor \\
Elezi \etal \cite{elezi2016game} & 2016 & Gamification & CodeArena  \\
Haendler \& Neumann \cite{haendler2019serious} & 2019 & Gamification & N/A  \\
Haendler \etal \cite{haendler2019refactutor} & 2019 & Tutoring system & refacTutor \\
Haendler \etal \cite{haendler2019interactive} & 2019 &  Tutoring system & refacTutor \\
Keuning \etal \cite{keuning2020student} & 2020 & Tutoring system & refacTutor \\
Keuning \etal \cite{keuning2021tutoring} & 2021 & Tutoring system & refacTutor \\
Izu \etal \cite{izu2022resource} & 2022 & Experimentation & N/A \\
\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\vspace{-.3cm}
\end{table}

%\begin{comment}

\begin{table}
  \centering
  %\fontsize{8}{9}\selectfont
	%\tabcolsep=0.05cm
	 \caption{Related work in code quality assessment tools.}
	 \label{Table:Related_Work_in_quality_tool}
%\begin{sideways}
\begin{adjustbox}{width=0.51\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lclllll}\hline
\toprule
\bfseries Tool & \bfseries Year &  \bfseries  Supported language &  \bfseries Detect smells? &  \bfseries Refactor? &  \bfseries Plugin? &  \bfseries Available?  \\
\midrule
Checkstyle \cite{Checkstyle} & 2001 & Java & No & No & No & Yes \\
Pylint \cite{Pylint} & 2001 &  Python & Yes & Yes & No & Yes \\
Style++ \cite{ala2004supporting} & 2004  & C++ & No & No & No & No \\
PMD \cite{PMD} & 2005 & Java & Partly & No & Yes & Yes\\
%SonarQube \cite{SonarQube} & 2006 & \\
FindBugs/SpotBugs \cite{FindBugs} & 2006  & Java & No & No & Yes & Yes  \\
\textbf{JDeodorant} \cite{tsantalis2008jdeodorant} & \textbf{2007}  & \textbf{Java} & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} \\
Java Critiquer \cite{qiu2008incremental} & 2008 & Java & No & No & No & No \\
Flack8 \cite{flake8} & 2010  & Python & No & No & Yes & Yes \\ 
%Codacy & & Quality \& security & \\
%Qodana & & Quality \& security & \\
CodeRush \cite{CodeRush} & 2012 & .NET & No & Yes & Yes & Trial\\
Refaster/Error Prone \cite{wasserman2013scalable} & 2013 & Java & No & Yes & No & Yes \\
FrenchPress \cite{blau2015frenchpress} & 2015  & Java & No & No & Yes & No \\
ReSharper \cite{ReSharper} & 2015 & .NET & Yes & Yes & Yes & Trial \\
RefactorIT \cite{RefactorIT} & 2015 & Java & No & Yes & Yes & Trial \\
FaultBuster \cite{szHoke2015faultbuster} & 2015 & Java & Yes & Yes & Yes & No \\
AutoStyle \cite{roy2016scale} & 2016  & Python, Java, Ruby & No & No & No & No\\
WebTA \cite{ureel2019automated} & 2019  & Java & No & No & No & No \\
Tutor  \cite{keuning2021tutoring} & 2021  & Java & No & No & No & Yes\\
Hyperstyle \cite{birillo2022hyperstyle} & 2022 & Python, Java, JavaScript, Kotlin  & No & No & No & Yes  \\ 



\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\vspace{-.3cm}
\end{table}
%\end{comment}
